Bayes Optimal Informer Sets for Early-Stage Drug Discovery

An important experimental design problem in early-stage drug discovery is how to prioritize available compounds for testing when very little is known about the target protein. Informer based ranking (IBR) methods address the prioritization problem when the compounds have provided bioactivity data on other potentially relevant targets. An IBR method selects an informer set of compounds, and then prioritizes the remaining compounds on the basis of new bioactivity experiments performed with the informer set on the target. We formalize the problem as a two-stage decision problem and introduce the Bayes Optimal Informer SEt (BOISE) method for its solution. BOISE leverages a flexible model of the initial bioactivity data, a relevant loss function, and effective computational schemes to resolve the two-step design problem. We evaluate BOISE and compare it to other IBR strategies in two retrospective studies, one on protein-kinase inhibition and the other on anti-cancer drug sensitivity. In both empirical settings BOISE exhibits better predictive performance than available methods. It also behaves well with missing data, where methods that use matrix completion show worse predictive performance. We provide an R implementation of BOISE at https://github.com/wiscstatman/esdd/BOISE

==> extra.tex <==


\begin{figure}[!ht]
\centering
\includegraphics[width=5.0in]{DPMM_performance.png}
\caption{\label{fig:mcmc} 
{\bf Mixing properties of MCMC sampling over clusters on PKIS1 and GDSC} The plots are based on the chain over numbers of clusters in each DPMM sample.}
\end{figure}


Intuitively, having more intermediate data should tend to reduce the risk, and calculations confirm:
\begin{theorem}
For two sets $A\subset B\subset J$, we have:
${\mbox {\rm PEL}}_1(x_0,A) \geq {\mbox {\rm PEL}}_1(x_0,B)$.
\end{theorem}

{\bf Miscellaneous}


If we let $\Phi = \{\phi_1,\cdots,\phi_K\}$ be the distinct parameters in~(\ref{eq:modelstructure}), the posterior mass of $\mathcal C$ given $x_0$ is:
\begin{align*}
    p(\mathcal C|x_0) &\propto p(x_0|\mathcal C)p(\mathcal C)\\
     &= \{\int \prod_{k=1}^K \prod_{i\in c_k} \, p(x_i\, |\, \phi_k)p(\Phi\,|\, \mathcal C) {\rm d}\Phi\} p(\mathcal C)\\
    &= \prod_{k=1}^K \, \int \{\prod_{i\in c_k}\prod_{j=1}^n  \phi_{k, j}^{x_{i,j}}(1-\phi_{k, j})^{1-x_{i,j}}p(\phi_{k,j}){\rm d}\phi_{k,j}\} \times p(\mathcal C).\\
&= \prod_{k=1}^K\prod_{j=1}^n \frac{B(\alpha_0+\sum_{i\in c_k} x_{i,j}, \beta_0+ m_k - \sum_{i\in c_k} x_{i,j })}{B(\alpha_0, \beta_0)} \times \frac{ m_0^K \Gamma(m_0) }{ \Gamma(m+m_0) } \prod_{k=1}^K
\Gamma( m_k ) .
\end{align*}

\section*{AC BOISE}

**maybe for a follow-up paper??**

The second method is a more heuristic one enlightened by decision tree. Recall that in ${\rm PEL}_1$ calculation procedure, the key step is formula~(\ref{eq:Posterior5}) that tells us how to calculate posterior expectation $\mathbb E(\theta_{i^*j}\,|\, \mathcal C, x_0,x_A)$, and this helps us think about the role that informer set $A$ plays in BOISE framework. Notice that~(\ref{eq:Posterior5}) consists of two parts: the posterior probability $p_k = P(i^*\in c_k\,|\,\mathcal{C},x_0,x_A)$, and another posterior expectation $E(\theta_{i^*j}\,|\, x_0,x_A,\mathcal{C},i^*\in c_k)$. We claim that informer set $A$ has little impact on the second part, since from expression~(\ref{eq:posterior3}) we can see that for $j\notin A$, informer set $A$ and intermediate data $x_A$ has nothing to do with $E(\theta_{i^*j}\,|\, x_0,x_A,\mathcal{C},i^*\in c_k)$, while for $j\in A$ we already know the interaction of $j$ on $i^*$ through intermediate data $x_A$ and hence we don't really need $E(\theta_{i^*j}\,|\, x_0,x_A,\mathcal{C},i^*\in c_k)$ in selecting top set $T^*(A,x_A,x_0)$. Therefore, informer set $A$ affects value of objective function ${\rm PEL}_1(x_0,A)$ mainly through posterior probability $p_k$. This observation suggests that the optimal informer set $A^*$ should give us an "optimal" posterior distribution $\{p_k,k=1,\cdots,K\}$, and hence we turn to entropy to define a "good" posterior distribution and find an approximate "best" informer set.  

Entropy is a measure of uncertainty associated with a random variable and is defined as expected bits required to communicate the value of this random variable:
\begin{eqnarray*}
H(Y) = -\int_y p(y)\log_2p(y)\,dy.
\end{eqnarray*}
Typically, less entropy means less uncertainty and is exactly what we desired. If we consider the cluster label of $i^*$ as a random variable $c(i^*)$, then the posterior distribution of $c(i^*)$ given $\mathcal C$, $x_A$ and $x_0$ is a multinomial distribution with $\{p_k,k=1,\cdots,K\}$ as event probabilities. In this way, we can define a "good" posterior distribution by its conditional entropy:
\begin{eqnarray}
\label{eq:Entropy}
H\left(c(i^*)\,|\,\mathcal{C},x_0,x_A\right) = -\sum_{k=1}^K p_k\log_2p_k
\end{eqnarray}
Using~(\ref{eq:Entropy}) we can score an informer set $A$ by its posterior expected entropy:
\begin{align}
    \label{eq:Score}
    \begin{split}
        \mathcal H(A) &= \mathbb E\left[H(c(i^*)\,|\,\mathcal{C},x_0,x_A)\,|\, x_0\right]\\
        &= \int_\mathbb{C} p(\mathcal{C}\,|\,x_0)\int_{x_A} p(x_A\,|\,x_0,\mathcal{C}) \, H\left(c(i^*)\,|\,\mathcal{C},x_0,x_A\right)\,dx_A\,d\mathcal{C}.
    \end{split}
\end{align}
and this is our approximate objective function for informer set selection. Our selected informer set $A^*$ should maintain a less posterior entropy $\mathcal H(A)$, and hence contain less uncertainty. 

The intuition for expression~(\ref{eq:Score}) is strongly connected with ID3 decision tree developed by Quinlan (1986): If we fix the original data $x_0$ and clustering assignment $\mathcal{C}$, then an ID3 decision tree algorithm aims for a split feature set $A\subset J$ that maximize the mutual information (or information gain):
\begin{eqnarray}
\label{eq:ID3}
{\rm MI}(x_0, A) = H(c(i^*)\,|\, \mathcal{C},x_0) - \int_{x_A} p(x_A\,|\,x_0,\mathcal{C})H(c(i^*)\,|\, \mathcal{C},x_0, x_A)\,dx_A.
\end{eqnarray}
Since $H(c(i^*)\,|\,\mathcal{C},x_0)$ is a constant when $\mathcal{C}$ and $x_0$ are given, maximizing ${\rm MI}(x_0, A)$ in~(\ref{eq:ID3}) is equivalent to minimizing the inner integral of $\mathcal H(A)$ in~(\ref{eq:Score}). It may worth to say that our approximate informer selection method is different from ID3 decision tree: our goal is not to predict the class label of $i^*$, as our clustering assignment is a random process on partitions. What we really need is a less chaotic system that can benefit our top set rule $T^*(A,x_A,x_0)$ and reduce the final loss $L(A^*,T^*)$. However, for the sake of easy understanding, our approximate informer selection method can be regarded as an ID3 decision tree algorithm with the same split feature of each level and maximum depth $n_A$. Also, we use ID3 decision tree algorithm instead of C4.5 algorithm (Quinlan 1993) since each candidate split feature $j\in J$ has the same number of possible outcomes: $0$ and $1$, so there is no bias towards features with more outcomes. Our second informer selection method is summarized in Algorithm \ref{Algo4}:

\begin{algorithm}
\caption{Accelerated Informer Selection}\label{Algo4}
\hspace*{\algorithmicindent} \textbf{Input:} Initial data $x_0$, size of informer set $n_A$, size of top set $n_T$.\\
\hspace*{\algorithmicindent} \textbf{Output:} Selected informer set of length $n_A$
\begin{algorithmic}[1]
\State \textbf{Initialization}: Let $A^* = \{\}$. Sample clustering assignments $\mathbb C$ from $p(\mathcal C\,|\, x_0)$ with Algorithm \ref{Algo1}.
\For{each $\mathcal C$ in $\mathbb C$}
    \State Sample $\mathbb{X}(\mathcal{C})$ from $p\left(x_{i^*}\,|\, \mathcal C,x_0\right)$ as in~(\ref{eq:Postphi}) and~(\ref{eq:Postc}).
    \Comment{\textbf{Auxiliary sample}}
\EndFor
\While{$|A^*| < n_A$}
    \For{each $j\in J\setminus A^*$}
        \For{each $\mathcal{C}$ in $\mathbb C$ and corresponding $\mathbb{X}(\mathcal{C})$}
            \State Evaluate $H(c(i^*)\,|\,\mathcal{C},x_0,x_{A^*\cup j})$ as in~(\ref{eq:Entropy});
        \EndFor
        \State Average over $x_{A^*\cup j}$ and $\mathcal{C}$ to get $\mathcal H(A^*\cup\{j\} )$ in~(\ref{eq:Score}). 
    \EndFor
    \State Let $A^*\gets A^*\cup \{j^*\}$, where $j^*$ is the minimizer of $\mathcal H(A^*\cup\{j\})$.
\EndWhile
\State Return $A^*$ as selected informer set.
\end{algorithmic}
\end{algorithm}
As mentioned in the beginning of this section, the major advantage of Algorithm \ref{Algo4} compared with Algorithm \ref{Algo3} is running time. In Algorithm \ref{Algo4} we bypass the computation of $\mathbb E\left(\theta_{ij}\,|\, x_0,x_A\right)$ and only use $p_k = P(i^*\in c_k\,|\, \mathcal C,x_0,x_A)$ to select informer set. This can improve our BOISE running time from days to hours while still maintaining similar performance. Therefore, we name it as "Accelerated-BOISE" in our empirical analysis. Also, although Accelerated-BOISE uses different informer selection method as BOISE does, they both share the same top set rule $T^*(A,x_A,x_0)$, which scores each $j\in J$ with their posterior expectation and choose the top $n_T$ as top set.  



\subsection{Proof of Theorem 2}
We first prove a lemma that will be used in proof of Theorem 2:
\begin{proposition}
In BOISE model (\ref{eq:modelstructure}), if we use $x_A$ and $x_k$ to denote subsets of outcomes on the new target: $x_{i^*A}$ and $x_{i^*k}$, and $x_{0A}$ and $x_{0k}$ to denote subsets of outcomes on the original data set $x_0$, then we have:
\begin{eqnarray}
\label{condition_ind}
x_A \indep x_k \, | \, x_0.
\end{eqnarray}
\end{proposition}

\begin{proof}[Proof of Proposition 1]
Notice that in model (\ref{eq:modelstructure}) we have:
\begin{align}
\label{condition_ind2}
\begin{split}
    (x_A,x_k) &\indep x_0 \, | \, (\theta_{i^*A},\theta_{i^*k});\\
x_A &\indep x_k \,|\, (\theta_{i^*A},\theta_{i^*k});\\
x_{0A} &\indep x_{0k} \,|\, (\theta_{i^*A},\theta_{i^*k});\\
\theta_{i^*A} &\indep \theta_{i^*k};\\
x_{0A} &\indep x_{0k}.
\end{split}
\end{align}
From independence and conditional independence in (\ref{condition_ind2}), we can show that $\theta_{i^*A}\indep \theta_{i^*k}\, | \, x_0$ as following:

\begin{align*}
    p(\theta_{i^*A},\theta_{i^*k}\,|\,x_0)&=
    \frac{p(x_0\,|\,\theta_{i^*A},\theta_{i^*k})p(\theta_{i^*A},\theta_{i^*k})}{p(x_0)}\\
    &= \frac{p(x_{0A},x_{0k}\,|\,\theta_{i^*A},\theta_{i^*k})p(\theta_{i^*A},\theta_{i^*k})}{p(x_{0A},x_{0k})}\\
    &= p(\theta_{i^*A}\,|\,x_{0A})p(\theta_{i^*k}\,|\,x_{0k})\\
    &= p(\theta_{i^*A}\,|\,x_0)p(\theta_{i^*k}\,|\,x_0).
\end{align*}

Therefore, for desired $p(x_A,x_k\,|\,x_0)$ we have:
\begin{align}
\begin{split}
    p(x_A,x_k\,|\,x_0) &= \int_\Theta p(x_A,x_k\,|\,\theta_{i^*A},\theta_{i^*k},x_0)p(\theta_{i^*A},\theta_{i^*k}\,|\,x_0) {\rm d}\theta_{i^*A}{\rm d}\theta_{i^*k}\\
    &= \int_\Theta p(x_A\,|\,\theta_{i^*A})p(x_k\,|\,\theta_{i^*k})p(\theta_{i^*A}\,|\,x_0)p(\theta_{i^*k}\,|\,x_0){\rm d}\theta_{i^*A}{\rm d}\theta_{i^*k}\\
    &= p(x_A\,|\,x_0)p(x_k\,|\,x_0).
\end{split}
\end{align}
and this is equivalent to $x_A \indep x_k \, | \, x_0$.
\end{proof}

With the help of Proposition 1 we can now prove Theorem 2:

\begin{proof}[Proof of Theorem 2]

When $x_0$ is given, we can write ${\mbox {\rm PEL}}_1(x_0,A)$ as ${\mbox {\rm PEL}}_1(A)$ for simplicity. To prove Theorem $2$ we only need to show that, for any set $A \subset J$, and any $k\notin A$, ${\mbox {\rm PEL}}_1(A\cup\{k\})\leq {\mbox {\rm PEL}}_1(A)$.

For simplicity of notation, we denote top set rule as 
$T_1^*(x_A,x_k) = T^*(A\cup\{k\}, x_{A\cup\{k\}}, x_0)$ and $T_2^*(x_A) = T^*(A, x_{A}, x_0)$. Recall that:
\begin{eqnarray*}
    {\mbox {\rm PEL}}_1(A\cup\{k\})= \int_{x_{A}}\int_{x_k} p\left( x_{A},x_k | x_0 \right) 
\left[ \sum_{j \in  T_1^*(x_A,x_k)}  1 - \mathbb{E} (\theta_{i^*,j} \, |\, x_0,x_A,x_k) \right]{\rm d}x_A {\rm d}x_k
\end{eqnarray*}
Here we still use $x_A$ and $x_k$ to denote $x_{i^*A}$ and $x_{i^*k}$, a subset of outcomes on the new target $i^*$.

From the fact that $T_1^*(x_A,x_k)$ is the Bayes rule when $A\cup\{k\}$, $x_{A\cup\{k\}}$ and $x_0$ are given, it should be no worse than $T_2^*(x_A)$ with regard to posterior expected loss, and hence we have:

\begin{align*}
&\int_{x_{A}}\int_{x_k} p\left( x_{A},x_k | x_0 \right)
\left[ \sum_{j \in  T_1^*(x_A,x_k)}  1 - \mathbb{E} (\theta_{i^*,j} \, |\, x_0,x_A,x_k) \right] {\rm d}x_A {\rm d}x_k\\
&\leq 
\int_{x_{A}}\int_{x_k} p\left( x_{A},x_k | x_0 \right)
\left[ \sum_{j \in  T_2^*(x_A)}  1 - \mathbb{E} (\theta_{i^*,j} \, |\, x_0,x_A,x_k) \right]{\rm d}x_A {\rm d}x_k
\end{align*}

From Proposition 1, $x_A \indep x_k \, | \, x_0$, and hence we have:

\begin{align*}
&\int_{x_{A}}\int_{x_k} p\left( x_{A},x_k | x_0 \right)
\left[ \sum_{j \in  T_2^*(x_A)}  1 - \mathbb{E} (\theta_{i^*,j} \, |\, x_0,x_A,x_k) \right]{\rm d}x_A {\rm d}x_k\\
    &= \int_{x_{A}}p\left(x_A|x_0\right)\sum_{j \in  T_2^*(x_A)}\left[\int_{x_k}p(x_k|x_0)\left(1-\mathbb{E} (\theta_{i^*,j} \, |\, x_0,x_A,x_k)\right){\rm d}x_k\right] {\rm d}x_A\\
&= \int_{x_{A}}p\left(x_A|x_0\right) \sum_{j \in  T_2^*(x_A)}\left[  1 - \mathbb{E} (\theta_{i^*,j} \, |\, x_0,x_A) \right]{\rm d}x_A.
\end{align*}


The first equality is because $T_2^*(x_A)$ is a function only of $x_A$. 

This implies ${\mbox {\rm PEL}}_1(A\cup\{k\})\leq {\mbox {\rm PEL}}_1(A)$, and the equality holds if and only if $T_1^*(x_A,x_k) = T_2^*(x_A)$, which means top sets are the same for any possible outcomes $x_A$ and $x_k$. 

\end{proof}

\subsection{Frequent hitters rule}

There are some researchers feeling that informer set is simply the most frequent hitters in compounds. We now show that even under the simplest setting frequent hitters may still not be the best informer set. 

Under our model (\ref{eq:modelstructure}), if we eliminate clustering structure for simplicity, that is:
\begin{eqnarray*}
&x_{i,j}|\theta_j \sim_{ind} {\rm Bernoulli}(\theta_j);\\
&\beta_j \sim_{i.i.d} {\rm Beta}(\alpha,\beta)
\end{eqnarray*}

Let $s_k = \sum_{i = 1}^n x_{ik}$ be column sums. We can assume that $s_1 \leq s_2 \leq~...~\leq s_m$.
The posterior distribution is:
\begin{eqnarray*}
\theta_j | x_0 \sim {\rm Beta}(\alpha + s_j, \beta + n - s_j)
\end{eqnarray*}
\begin{equation}
\theta_j|x_0,x_A \sim \left\{
\begin{aligned}
&{\rm Beta}(\alpha+s_j, \beta+n-s_j),{\rm if}~j\notin A,\\
&{\rm Beta}(\alpha+s_j+x_j^*, \beta+n+1-s_j-x_j^*),{\rm if}~j\in A,\\
\end{aligned}
\right.
\end{equation}

and the posterior expectation is:
\begin{equation}
E(\theta_j|x_0,x_A) = \left\{
\begin{aligned}
&(\alpha + s_j)/(\alpha + \beta + n),{\rm if}~j\notin A,\\
&(\alpha + s_j + x_j^*)/(\alpha + \beta + n +1),{\rm if}~j\in A,\\
\end{aligned}
\right.
\end{equation}

We first prove a general proposition:

\begin{proposition}
Given $n_A$, $n_T$ and the setting above, if for different informer sets $A_1$ and $A_2$, for any $0-1$ sequence $\nu$, $T^*(A_1, x_{A_1} = \nu,x_0) = \hat{T}(A_2,x_{A_2} = \nu,x_0) \equiv T$, i.e. Top set is constant w.r.t. any results of two different informer sets. Then ${\rm PEL}_1(x_0, A_1) = {\rm PEL}_1(x_0, A_2)$.
\end{proposition}

\begin{proof}
Let $\Omega = \{$All the 0-1 sequences of length $n_A \}$ be the sample space of $x_{A_1}$. Then from Fubini we have: 
\begin{align*}
    n_A - {\rm PEL}_1(x_0, A_1) &= \int_\Omega P(x_{A_1} = s|x_0)\sum_{j\in T} E(\theta_j|x_0, x_{A_1} = s) ~{\rm d}s\\
   &= \sum_{j\in T} \int_\Omega \int_{[0,1]} \theta_j \times \frac{P(\theta_j,x_0,x_{A_1}=s )}{P(x_0,x_{A_1} = s)}\times \frac{P(x_{A_1} = s, x_0)}{P(x_0)}~{\rm d}\theta_j~{\rm d}s\\
    &= \sum_{j \in T} \int_{[0,1]}\int_\Omega \theta_j P(\theta_j, x_{A_1} = s|x_0) ~{\rm d}s~{\rm d}\theta_j\\
    &= \sum_{j\in T}E(\theta_j|x_0)
\end{align*}

Since the value of ${\rm PEL}_1(x_0,A_1)$ has nothing to do with informer set $A_1$, ${\rm PEL}_1(x_0, A) \equiv {\rm Constant}$ for any informer sets.
\end{proof}

When there are no ties in $s_j$'s, we can show that ${\rm PEL}_1(x_0, A)$ is constant risk for any $A$ under this simple setting:

Since
$$
E(\theta_i|x_0, x_i^* = 0, x_k^* = 1) \geq
E(\theta_k|x_0,x_i^* = 0, x_k^* = 1), {\rm for}~k < i;
$$

and
$$
E(\theta_i|x_0, x_j^*, x_k^* = 1) > E(\theta_k|x_0,x_j^*, x_k^* = 1), {\rm for}~k < i, j \neq i,k.
$$

This means: When there is no ties, $E(\beta_i|x_0, x_A) \geq E(\beta_k|x_0, x_A)$ for any $k < i$ and $x_A$. Therefore, we will choose a constant top set $T = \{m-n_T+1,~...,~m-1,~m\}$ w.r.t any informer set $A$ and any results of $x_A$. 

From our previous Proposition, when there is no ties, Top set is constant w.r.t. any results of different informer sets, and hence ${\rm PEL}_1(x_0, A)$ is a constant for any A. 

We now show that: when $n_A = 1$, $n_T = 2$, and $s_m > s_{m-1} = s_{m-2}$, $A^* = \{m-1\}$ is better than the Frequent Hitters Rule $\hat{A} = \{m\}$ in our framework.

First calculate $P(x_A|x_0)$:
\begin{align*}
    P(x_A|x_0) 
    &= \int_\Theta P(x_A|\theta_1,...,\theta_m)P(\theta_1,...,\theta_m|x_0){\rm d}\theta\\
    &= \int_{\Theta_A} P(x_A|\theta_A)P(\theta_A|x_0){\rm d}\beta_A\\
    &= \frac{1}{\alpha+\beta+n}\times\frac{\Gamma(\alpha+s_A+x_A)\Gamma(\beta+n+1-x_A-s_A))}{\Gamma(\alpha+s_A)\Gamma(\beta+n-s_A)}
\end{align*}

Next calculate ${\rm PEL}_1(x_0,A)$:

Recall $\hat{A} = \{m\}$ and $A^* = \{m-1\}$. Notice that whenever $x_{\hat{A}} = 0~ {\rm or} ~1$, $T^*(x_0,x_{\hat{A}},x_0) = \{m-1,m\}$. 

\begin{align*}
    n_T - {\rm PEL}_1(x_0, \hat{A}) &= P(x_m^* = 1|x_0)\left[E(\theta_m|x_0,x_m^* = 1) + E(\theta_{m-1}|x_0, x_m^* = 1)\right] +\\ &~~~~P(x_m^* = 0|x_0)\left[E(\theta_m|x_0,x_m^* = 0) + E(\theta_{m-1}|x_0, x_m^* = 0)\right]\\
    &= \frac{(\alpha + s_m) + (\alpha+s_{m-1})}{\alpha+\beta+n}
\end{align*}

When $x_{A^*} = 1$, $T^*(x_0,x_{A^*},x_0) = \{m-1,m\}$; When $x_{A^*} = 0$,
we have $T^*(x_0,x_{A^*},x_0) = \{m,m-2\}$.

\begin{align*}
    n_T - {\rm PEL}_1(x_0, A^*) &= P(x_{m-1}^* = 1|x_0)\left[E(\theta_m|x_0,x_{m-1}^* = 1) + E(\theta_{m-1}|x_0, x_{m-1}^* = 1)\right] +\\ &~~~~P(x_{m-1}^* = 0|x_0)\left[E(\theta_m|x_0,x_{m-1}^* = 0) + E(\theta_{m-2}|x_0, x_{m-1}^* = 0)\right]\\
    &= \frac{\alpha + s_m}{\alpha+\beta+n} + \frac{\alpha+s_{m-1}}{\alpha+\beta+n}(\frac{\alpha+s_{m-1}+ 1}{\alpha+\beta+n+1} + \frac{\beta+n-s_{m-1}}{\alpha+\beta+n})
\end{align*}

Since:
$$
\frac{\alpha+s_{m-1}+1}{\alpha+\beta+n+1} > \frac{\alpha+s_{m-1}}{\alpha+\beta+n}.
$$

We have 
$n_T - {\rm PEL}_1(x_0, \hat{A}) <n_T - {\rm PEL}_1(x_0, A^*)$, 
so $\hat{A}$ is not the Bayes rule.


\section*{Tables} \label{sec:tab}
\addcontentsline{toc}{section}{Tables}



\clearpage

\section*{Figures} \label{sec:fig}
\addcontentsline{toc}{section}{Figures}

\begin{figure}[hp]
  \centering
  \includegraphics[width=.6\textwidth]{../fig/placeholder.pdf}
  \caption{Placeholder}
  \label{fig:placeholder}
\end{figure}



\subsection{Prospective Results}
We apply BOISE and Accelerated-BOISE on three novel kinase targets not included in PKIS1 target sets. They are microbial targets and hence phylogenetically distant from most human protein kinase contained in PKIS1 data set. These three new targets are PknB (\textit{Mycobacterium tuberculosis} kinase), BGLF4 (\textit{Epstein-Barr virus} kinase) and ROP18 (\textit{Toxoplasma gondii} kinase). 

The task for informer based ranking methods is to prioritize which PKIS1 compounds might be active on these three targets with the inhibition value obtained on an informer set of size $16$. These targets are already screened in advance, yet the screening data are held separately from all methods before informer selection. After selecting the informer compounds, screening data only for those selected informer compounds are provided to each method to rank the whole compound set. To evaluate the performance of different methods, all of the available PKIS1 compounds are tested, and different methods are compared with respect to numbers of hits recovered in their top $10\%$ of ranked compounds for all three targets. Based on the screening results, the active thresholds defined by 2SD criteria~(\ref{eq:thresh}) are: $13.4\%$ for PknB, $20.2\%$ for BGLF4 and $43.8\%$ for ROP18.

However, these experimentally determined thresholds contain information from non-informer compounds and should be kept away from all methods. In order to binarize the inhibition values to get the intermediate data $x_A$ for BOISE and Accelerated-BOISE, we focus on the sub-matrix of inhibition data $Z$ on informer compounds, say $Z_A$, and keep track of all the possible binary outcomes $x_l$ of each row of $Z_A$. For rows with same binary outcome $x_l$, we compute a centroid corresponding to this outcome, say $c_l$, then the binary outcome $x_A$ of new target with inhibition values $z_A$ is defined as:
\begin{align}
    \label{eq:Code}
    \begin{split}
        x_A &= x_{l^*} \\
        s.t.\,~ ||z_A - c_{l^*}|| &= \argmin\limits_{l} ||z_A-c_l||
    \end{split}
\end{align}
Procedure~(\ref{eq:Code}) is exactly the same as CS and AS. There may be better ways to derive intermediate data, however, we follow the same procedure since we want to show our better performance comes from BOISE and Accelerated-BOISE themselves but not from a more accurate intermediate data. The result is summarized in following Table 1:
\bigskip
\begin{table}[ht!]
\centering
\caption{\label{tbl:t1}
{\bf Recovery counts by different informer based ranking methods on new kinase targets PknB, BGLF4 and ROP18 using PKIS1 data set.}}

\begin{tabular}{ ccccccccc }
\multicolumn{2}{l}{} & \multicolumn{2}{c}{Baselines} & \multicolumn{5}{c}{Non-baselines} \\
\multicolumn{1}{c}{Targets} & \multicolumn{1}{c}{Matrix} & \multicolumn{1}{c}{BC\textsubscript{w}} & \multicolumn{1}{c}{BF\textsubscript{w}} & \multicolumn{1}{c}{RS} & 
\multicolumn{1}{c}{CS} & 
\multicolumn{1}{c}{AS} & 
%\multicolumn{1}{c}{AC-BOISE} &
\multicolumn{1}{c}{BOISE} & \multicolumn{1}{c}{total} \\
 \hline
 PKnB & PKIS1 & 1 & 7 & 7 & 2& 3 & \textbf{7}  & 8 \\
 BGLF4 & PKIS1 & 3 & 9 & 3 & 7 & 10 & \textbf{10}  & 11 \\
 ROP18 & PKIS1 & 4 & 7 & 4 & 4 & 2 & \textbf{7}  &16 \\
\end{tabular}\\
\end{table}
\bigskip

In Table 1, the total number of experimentally determined active compounds is indicated in the \textit{total} column. The values below each of the methods indicate the number of experimentally determined active compounds that were ranked in the top $10\%$ of predicted active compounds by each method. 

It can be shown that RS, CS or AS can be better than baseline methods ${\rm BF}_w$ on some targets, but fail to beat the baseline on others, however, BOISE are consistently better than baseline and RS, AS and CS methods on all 3 new targets. It may worth to say that baseline method is performing pretty well on these three new targets for two reasons: One is that baselines are allowed to utilize chemical structure similarity information of compounds in ranking, while non-baseline methods are not allowed to use addition information except inhibition matrix. The other is, as stated earlier, these three targets are all microbial targets that are far away from targets in PKIS1 phylogenetically. Therefore, inhibition data in PKIS1 is less informative than chemical structure similarity on these three targets, and $(7,10,7)$ recovery seems to be the best informer based ranking methods can do with PKIS1 data set. We can see a more significant difference among baseline methods, RS/CS/AS methods, and BOISE in a retrospective analysis still on PKIS1.


\section{D: Baseline IBR strategies}
\textcolor{blue}{**we may need to drop this section for space in ENAR submission (good for thesis!!)**}
We compare BOISE with $5$ previous IBR strategies: Regression Selection (RS), Coding Selection (CS), Adaptive Selection (AS), as well as $2$ baseline methods using chemical structure information: Baseline Chemometric (BC) and Baseline Frequent-hitters (BF) (Zhang {\em et al.} 2019).

Like BOISE, RS, CS, and AS all use only the interaction matrix to select informers and rank compounds. RS applies k-means clustering on the continuous interaction data and uses a penalized multinomial logistic regression to select informers; CS is based on binary interaction data. It treats the $0$-$1$ string as a ``code" and selects informer by distance between these codes; AS applies k-means on the continuous interaction data, selects an initial informer set with group LASSO (Yuan and Lin 2006), and augments the informer set by minimizing the distance between informers and non-informers.

The chemical baseline IBR methods use both the interaction matrix and chemical structure data on compounds. These methods include $2$ informer set selection methods and $3$ ranking methods. 

Informer set selection methods include BC and BF: BC is based on chemical structural diversity of compounds denoted by RDKit-derived Morgan chemical fingerprints. It applies hierarchical clustering on Jaccard distance matrix of Morgan fingerprints. The cluster centroids are selected as informer set;
BF is based on binary bioactivity matrix. After ranking compounds by how many active targets they have, we select compounds with most active targets as the informer set.

As for ranking methods, simple expansion (-s) is to rank each non-informer compound by its  distance to the nearest active informer compound based on Jaccard distance of Morgan fingerprints; loop expansion (-l) is to first order all active informer compounds by their hit frequency, then iteratively assign non-informer compounds to each active informer compound, one at a time, based on Jaccard distance of Morgan fingerprints; weighted expansion (-w) is to rank each non-informer compound by a specific score. The score is defined as the inner product between the vector of binary bioactivity on informer compounds and the vector of Jaccard similarity to informer compounds.
\tony{If you keep this appendix, it looks like a lot of the baseline text can be cut.  Did you only run the -w version here?  If so, -s and -l aren't needed in the description.}

\peng{-s and -l are also running on PKIS1, it's not shown on plots for space reasons.. Yeah I can remove -s and -l. Thanks!}
%In practice, BF method is better than BC method, and all $3$ ranking methods perform similarly, with weighted expansion slightly better than other $2$ methods. 


\section{MCC/F1 metrics and previous t-test evaluations}

For each IBR method and evaluation metric, we conduct the pairwise comparison of whether ${\rm IBR} - {\rm BOISE} = 0$. After controlling overall Type-I error under $5\%$, we get the mean difference between all IBR methods and BOISE less than $0$ under all metrics and both $n_A$ values: Under NEF10 criteria, the closest difference is $-0.063$ when $n_A = 8$ and $-0.042$ when $n_A = 16$. Under ROCAUC criteria, the cloest difference is $-0.031$ when $n_A = 8$ and $-0.029$ when $n_A = 16$. 

Same thing happens when we boost informer set size from $n_A = 8$ to $16$. We rely on distributed computing offered by CHTC to complete this cross validation as BOISE will take a lot of time on personal computer. Empirical results summarized in Figure \ref{fig:pkis16} show that BOISE and AC-BOISE are still significantly better than previous methods: Under NEF10 metric, Adaptive Selection (AS16) is the best method other than (AC-)BOISE and the paired t-test shows that the mean difference between BOISE and AS is $0.0421$ with p-value $=6.115\times 10^{-7}$;  Under ROCAUC metric, Regression Selection (RS16) is the best method other than (AC-)BOISE and the paired t-test shows that the mean difference between BOISE and RS is $0.0294$ with p-value $=1.303\times 10^{-4}$. 

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=5.0in]{PKIS1_16_eval.png}
% \caption{\label{fig:pkis16} 
% {\bf Violin plot comparison of different methods under informer size $n_A =16$ with respect to compound ranking performance assessed by NEF10 and ROCAUC.}}
% \end{figure}


%%%%% Below is about MCC/F1 results (new metrics) %%%%%
Moreover, there are some concerns about ROCAUC metric, saying that it will amplify the scores. To address these concerns, we include other well-known classification criteria like Matthews Correlation Coefficient (MCC) and F1 Score into our comparison. It turns out different criteria will do no harm to BOISE superiority. 
Recall that definition of MCC is:
\begin{eqnarray}
\label{eq:mcc}
MCC = \frac{TP\times TN-FP\times FN}{\sqrt{(TP+FP)(TP+FN)(TN+FP)(TN+FN)}}
\end{eqnarray}

and definition of F1 Score is:
\begin{eqnarray}
\label{eq:F1}
F1 = \frac{2TP}{2TP+FN+FP}
\end{eqnarray}
where TP, FP, TN, FN come from confusion matrix. MCC takes value in $[-1,1]$, with MCC of $0$ indicates a random guess; F1 Score takes value in $[0,1]$, with F1 Score of $0.5$ indicates a random guess. Notice that MCC and F1 Score are both for binary classification, yet we are doing ranking for compounds, we will just choose the best split point for our ranked compounds to calculate the classification criteria. 

\begin{figure}[!ht]
\centering
\includegraphics[width=5.0in]{PKIS1_8_mccf1.png}
\caption{\label{fig:mcc} 
{\bf Violin plot comparison of different methods under informer size $n_A =8$ with respect to performance assessed by Matthews Correlation Coefficient (MCC) and F1 Score.} }
\end{figure}


Figure \ref{fig:mcc} shows that (AC)-BOISE are still best under these classification criteria: Adaptive Selection (AS8) is the best method other than (AC)-BOISE  under MCC and F1 Score. When caring about MCC, the mean difference between AS8 and BOISE8 is is $0.0436$ with p-value $=3.722\times 10^{-6}$; and  mean difference between AS8 and AC-BOISE8 is $0.0401$ with p-value $=2.839\times 10^{-5}$; When caring about F1 Score, the mean difference between AS8 and BOISE is $0.0480$ with p-value $=1.637\times 10^{-6}$; and  mean difference between AS8 and AC-BOISE is $0.0433$ with p-value $=1.783\times 10^{-5}$.

\section{Old intro of DPMM}
Dirichlet process mixture model (DPMM) origins from Antoniak (1974) and Ferguson (1983). It can be handled in a Bayesian framework by employing Dirichlet process as prior distribution on mixing proportions. DPMM computations have become feasible via MCMC methods for sampling from the posterior distribution of parameters corresponding to distribution of each cluster and of the associations of mixture components with observations. In particular, when conjugate prior distributions are used, algorithms based on Gibbs sampling can easily be implemented for DPMM.

A general form of DPMM is:
\begin{align}
    x_i\, | \, \theta_i &\sim F(\theta_i);\\
    \theta_i\, |\, G &\sim G;\\
    G &\sim DP(G_0,m_0).
\end{align}

Ferguson (1973) has shown measures drawn from a Dirichlet process~(\ref{eq:DPMM}) are discrete with probability $1$, therefore DPMM can be seen as countably infinite mixtures. Also, we can see that draws from Dirichlet process are both discrete and exhibit a clustering property through P\'{o}lya urn scheme (Blackwell and MacQueen 1973): Suppose $\theta_1,\theta_2,\cdots$ is a sequence of i.i.d random variables distributed with respect to $G$, then successive conditional distribution of $\theta_i$ given previous $\theta_1, \theta_2,\cdots,\theta_{i-1}$ can be derived by integrating $G$ out in model~(\ref{eq:DPMM}):
\begin{eqnarray}
\label{eq:Urn}
    \theta_i\,|\, \theta_1,\cdots,\theta_{i-1},m_0,G_0 \, \sim\, \frac{1}{i-1+m_0}\sum_{j=1}^{i-1}\delta(\theta_j) + \frac{m_0}{i-1+m_0}G_0
\end{eqnarray}
where $\delta(\theta_j)$ is the probability measure concentrated on single point $\theta_j$. 

This conditional distribution shows that $\theta_i$ has positive probability of being equal to one of the previous draws and there is a clustering tendency: the more one point is drawn in the past, the more often it will be drawn in the future. It can be shown more clear by re-parameterization: Let $\phi_1,\phi_2,\cdots,\phi_K$ be the distinct values in $\theta_1,\theta_2,\cdots,\theta_{i-1}$ and $m_k = \sum_{j<i} \mathbbm{1}(\theta_j=\phi_k)$ be the number of $\theta_j$ that is equal to $\phi_k$, then previous conditional distribution~(\ref{eq:Urn}) can be rewritten as:

\begin{eqnarray}
    \theta_i\,|\, \theta_1,\cdots,\theta_{i-1},m_0,G_0 \, \sim\, \sum_{k=1}^{K}\frac{m_k}{i-1+m_0}\delta(\phi_k) + \frac{m_0}{i-1+m_0}G_0
\end{eqnarray}
this is the Chinese Restaurant (CR) process (Aldous 1985) we used in BOISE. We can interpret conditional distribution~(\ref{eq:CR}) in terms of a Chinese restaurant with an infinite number of tables: Imagine each $\phi_k$ is a table and each $\theta_i$ is the $i$th customer. When $i$th customer coming into the restaurant, he will sit at table $k$ with probability $\frac{m_k}{m_0+i-1}$ and sit at a brand new table with probability $\frac{m_0}{m_0+i-1}$. This process will generate a clustering on $m$ customers and is an efficient representation of Dirichlet process. The Chinese restaurant process implies we can write DPMM in a limiting form with latent cluster labels $c$ (Neal 2000):

\begin{align}
\label{eq: DPMM2}
\begin{split}
    x_i\,|\,c,\phi &\sim F(\phi_{c(i)});\\
    c(i)\,|\,p &\sim {\rm Discrete}(p_1,\cdots,p_K);\\
    \phi_c &\sim G_0;\\
    p_1,\cdots,p_K &\sim {\rm Dirichlet}(\frac{m_0}{K},\cdots,\frac{m_0}{K})
\end{split}
\end{align}
Note that we use $c(i)$ to denote cluster label of $i$-th target, $i = 1,2,\cdots,m$, and $c_k$ to denote indices of targets that fall in $k$-th cluster, $k=1,2,\cdots,K$. $c(i) = k$ if and only if $i \in c_k$. When $K\to \infty$ the conditional distribution $c(i)\,|\,c(1),\cdots,c(i-1)$ will approximate a Chinese restaurant process, and model~(\ref{eq: DPMM2}) is equivalent to~(\ref{eq:DPMM}). By taking the limit, the posterior distribution of $c(i)$ given all other cluster labels $c(-i)$, observation $x_i$ and parameters corresponding to existing clusters $\Phi = (\phi_1,\cdots,\phi_K)$ is:

\begin{equation}
P(c(i) = k\,|\, c(-i), x_i, \Phi) \propto \begin{cases}
		\frac{m_{-i,k}}{m-1+m_0}F(x_i,\phi_k), &\text{ if }
	    \exists \, c(j) = k, j\neq i\\
		\frac{m_0}{m-1+m_0}\int F(y_i,\phi)dG_0(\phi). & \text{ if }
		\nexists \, c(j)= k, j \neq i.
	\end{cases}
\end{equation}
this posterior distribution leads to our final Gibbs sampler in Algorithm \ref{Algo1}.

Dirichlet process mixture model (DPMM) is a powerful tool for clustering data that enables the inference of a countably infinite number of mixture components. With countably infinite mixtures we bypass the assumption that the correct number of clusters is "known". Detailed introduction of DPMM is enclosed in Supplementary materials.
Generally speaking, DPMM applies to data $x_1,\cdots,x_n$ which are regarded as exchangeable. The distribution from which $x_i$ is sampled can be parameterized as a mixture of distributions of the form $F(\theta)$, and the mixing distribution of $\theta$ is $G$. Typical choice of prior for mixing distribution $G$ is a Dirichlet process with base distribution $G_0$ and prior mass $m_0$. 
